Evaluating LLMs for Hardware Design and Test

Large Language Models (LLMs) have demonstrated capabilities for producing code in Hardware Description Languages (HDLs). However, most of the focus remains on their abilities to write functional code, not test code. The hardware design process consists of both design and test, and so eschewing validation and verification leaves considerable potential benefit unexplored, given that a design and test framework may allow for progress towards full automation of the digital design pipeline. In this work, we perform one of the first studies exploring how a LLM can both design and test hardware modules from provided specifications. Using a suite of 8 representative benchmarks, we examined the capabilities and limitations of the state-of-the-art conversational LLMs when producing Verilog for functional and verification purposes. We taped out the benchmarks on a Skywater 130nm shuttle and received the functional chip.

==> fig/gpt3p5-results.tex <==
\setlength\tabcolsep{2pt} % default value: 6pt
\resizebox{\linewidth}{!}{%
\begin{tabular}{l|l|l|l|l}
\hline
Benchmark                           & Test Set & Outcome & Accurate & \# Messages \\ \hline
\multirow{3}{*}{Shift Register}     & T1       & TF      & \cmark          & 3           \\ \cline{2-5}
                                    & T2       & TF      & \cmark          & 9           \\ \cline{2-5}
                                    & T3       & AHF     & \cmark          & 15          \\ \hline
\multirow{3}{*}{Sequence Generator} & T1       & AHF     & \cmark          & 14          \\ \cline{2-5}
                                    & T2       & TH      & \cmark          & 4           \\ \cline{2-5}
                                    & T3       & AHF     & \cmark          & 20          \\ \hline
\multirow{3}{*}{Sequence Detector}  & T1       & FAIL    & -          & 24          \\ \cline{2-5}
                                    & T2       & SHF     & \cmark          & 9           \\ \cline{2-5}
                                    & T3       & TF      & \cmark          & 13          \\ \hline
\multirow{3}{*}{ABRO}               & T1       & FAIL    & -          & 16          \\ \cline{2-5}
                                    & T2       & AHF     & \cmark          & 20          \\ \cline{2-5}
                                    & T3       & TF      & \cmark          & 12          \\ \hline
\multirow{3}{*}{LFSR}               & T1       & TF      & \cmark          & 12          \\ \cline{2-5}
                                    & T2       & SHF     & \cmark          & 7           \\ \cline{2-5}
                                    & T3       & SHF     & -          & 9           \\ \hline
\multirow{3}{*}{Binary to BCD}      & T1       & TF      & \cmark          & 4           \\ \cline{2-5}
                                    & T2       & NF      & \cmark          & 2           \\ \cline{2-5}
                                    & T3       & SHF     & \cmark          & 9           \\ \hline
\multirow{3}{*}{Traffic Light}      & T1       & TF      & \cmark          & 4           \\ \cline{2-5}
                                    & T2       & SHF     & \cmark          & 12          \\ \cline{2-5}
                                    & T3       & TF      & \cmark          & 5           \\ \hline
\multirow{3}{*}{Dice Roller}        & T1       & SHF     & \xmark          & 8           \\ \cline{2-5}
                                    & T2       & SHF     & \cmark          & 9           \\ \cline{2-5}
                                    & T3       & SHF     & \xmark          & 18          \\ \hline
\end{tabular}
}


==> fig/gpt4-results.tex <==
\setlength\tabcolsep{2pt} % default value: 6pt
\resizebox{\linewidth}{!}{%
\begin{tabular}{l|l|l|l|l}
\hline
Benchmark                           & Test Set & Outcome & Accurate & \# Messages \\ \hline
\multirow{3}{*}{Shift Register}     & T1       & TF      & \cmark          & 3           \\ \cline{2-5}
                                    & T2       & TF      & \cmark          & 9           \\ \cline{2-5}
                                    & T3       & AHF     & \cmark          & 15          \\ \hline
\multirow{3}{*}{Sequence Generator} & T1       & AHF     & \cmark          & 14          \\ \cline{2-5}
                                    & T2       & TH      & \cmark          & 4           \\ \cline{2-5}
                                    & T3       & AHF     & \cmark          & 20          \\ \hline
\multirow{3}{*}{Sequence Detector}  & T1       & FAIL    & -          & 24          \\ \cline{2-5}
                                    & T2       & SHF     & \cmark          & 9           \\ \cline{2-5}
                                    & T3       & TF      & \cmark          & 13          \\ \hline
\multirow{3}{*}{ABRO}               & T1       & FAIL    & -          & 16          \\ \cline{2-5}
                                    & T2       & AHF     & \cmark          & 20          \\ \cline{2-5}
                                    & T3       & TF      & \cmark          & 12          \\ \hline
\multirow{3}{*}{LFSR}               & T1       & TF      & \cmark          & 12          \\ \cline{2-5}
                                    & T2       & SHF     & \cmark          & 7           \\ \cline{2-5}
                                    & T3       & SHF     & \cmark          & 9           \\ \hline
\multirow{3}{*}{Binary to BCD}      & T1       & TF      & \cmark          & 4           \\ \cline{2-5}
                                    & T2       & NF      & \cmark          & 2           \\ \cline{2-5}
                                    & T3       & SHF     & \cmark          & 9           \\ \hline
\multirow{3}{*}{Traffic Light}      & T1       & TF      & \cmark          & 4           \\ \cline{2-5}
                                    & T2       & SHF     & \cmark          & 12          \\ \cline{2-5}
                                    & T3       & TF      & \cmark          & 5           \\ \hline
\multirow{3}{*}{Dice Roller}        & T1       & SHF     & \xmark          & 8           \\ \cline{2-5}
                                    & T2       & SHF     & \cmark          & 9           \\ \cline{2-5}
                                    & T3       & SHF     & \xmark          & 18          \\ \hline
\end{tabular}
}


==> fig/isa.tex <==
\resizebox{\linewidth}{!}{\begin{tabular}{|l|p{6cm}|c|}
\hline
\textbf{Instruction} & \textbf{Description}                         & \textbf{Opcode} \\ \hline
\multicolumn{3}{|c|}{\textbf{Instructions with Immediate Operands}} \\ \hline
ADDI        & Add immediate to Accumulator        & 1110XXXX        \\ \hline
\multicolumn{3}{|c|}{\textbf{Instructions with Variable-Data Operands}} \\ \hline
LDA         & Load Accumulator with memory contents      & 000MMMMM            \\ \hline
STA         & Store Accumulator to memory                & 001MMMMM            \\ \hline
ADD         & Add memory contents to Accumulator         & 010MMMMM            \\ \hline
SUB         & Subtract memory contents from Accumulator  & 011MMMMM            \\ \hline
AND         & AND memory contents with Accumulator       & 100MMMMM            \\ \hline
OR          & OR memory contents with Accumulator        & 101MMMMM            \\ \hline
XOR         & XOR memory contents with Accumulator       & 110MMMMM            \\ \hline
\multicolumn{3}{|c|}{\textbf{Control and Branching Instructions}} \\ \hline
JMP         & Jump to memory address                     & 11110000       \\ \hline
JSR         & Jump to Subroutine (save address to ACC)   & 11110001       \\ \hline
BEQ\_FWD    & Branch if ACC==0, forward (PC = PC + 3) & 11110010       \\ \hline
BEQ\_BWD    & Branch if ACC==0, backward (PC = PC - 2)& 11110011       \\ \hline
BNE\_FWD    & Branch if ACC!=0, forward (PC = PC + 3)& 11110100       \\ \hline
BNE\_BWD    & Branch if ACC!=0, backward (PC = PC - 2)& 11110101       \\ \hline
HLT         & Halt the processor until reset             & 11111111       \\ \hline
\multicolumn{3}{|c|}{\textbf{Data Manipulation Instructions}} \\ \hline
SHL         & Shift Accumulator left                                   & 11110110       \\ \hline
SHR         & Shift Accumulator right                                  & 11110111       \\ \hline
SHL4        & Shift Accumulator left by 4 bits                         & 11111000       \\ \hline
ROL         & Rotate Accumulator left                                  & 11111001       \\ \hline
ROR         & Rotate Accumulator right                                 & 11111010       \\ \hline
LDAR        & Load Accumulator via indirect mem. access M[ACC] & 11111011       \\ \hline
DEC         & Decrement Accumulator                                    & 11111100       \\ \hline
CLR         & Clear (Zero) Accumulator                                 & 11111101       \\ \hline
INV         & Invert (NOT) Accumulator                                 & 11111110       \\ \hline
\end{tabular}}

==> fig/msg_metadata.tex <==
\setlength\tabcolsep{2pt} % default value: 6pt
\resizebox{\linewidth}{!}{%
\begin{tabular}{|c|c|p{3.5cm}|c|c|c|c|c|c|}
\hline
\textbf{\begin{tabular}[c]{@{}l@{}}Cont.\\T. ID\end{tabular}} & \textbf{T. ID} & \textbf{Topic}               & \textbf{\begin{tabular}[c]{@{}l@{}}\# User\\ Msgs\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}\# \\ Restart\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}\# User\\ Lines\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}\# User\\ Chars\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}\# LLM\\ Lines\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}\# LLM\\ Chars\end{tabular}} \\ \hline

-            & \tikzmark{00}00              & Specification                & 22                                                          & 10                                                             & 45                                                               & 5025                                                             & 498                                                             & 44818                                                           \\ \hline

-             & 01              & Register specification       & 6                                                          & 2                                                              & 59                                                               & 4927                                                             & 91                                                              & 9961                                                            \\ \hline

-             & 02              & Shift registers and memory   & 5                                                          & 5                                                              & 65                                                               & 5444                                                             & 269                                                             & 9468                                                            \\ \hline

-             & \tikzmark{03}03              & Multi-cycle planning and ALU & 7                                                          & 2                                                              & 103                                                              & 7284                                                             & 243                                                             & 10148                                                           \\ \hline

-             & 04              & Control signal planning      & 13                                                          & 21                                                             & 216                                                              & 9205                                                             & 414                                                             & 20364                                                           \\ \hline

-             & 05              & Control Unit state logic     & 12                                                          & 11                                                             & 216                                                              & 9898                                                             & 742                                                             & 21663                                                           \\ \hline

-             & 06              & ISA to ALU opcode            & 4                                                           & 0                                                              & 72                                                               & 4576                                                             & 149                                                             & 5624                                                            \\ \hline

-             & \tikzmark{07}07              & Control unit output logic    & 11                                                          & 6                                                              & 266                                                              & 8632                                                             & 518                                                             & 19180                                                           \\ \hline

-             & \tikzmark{08}08              & Datapath components          & 12                                                          & 0                                                              & 144                                                              & 5385                                                             & 516                                                             & 15646                                                           \\ \hline

-             & 09              & Python assembler             & 3                                                           & 4                                                              & 127                                                              & 4231                                                             & 218                                                             & 6270                                                            \\ \hline

00\tikzmark{00d}             & 10             & Spec. branch update           & 1                                                           & 1                                                              & 14                                                               & 1275                                                             & 15                                                              & 1635                                                            \\ \hline

07\tikzmark{07d}            & \tikzmark{11}11             & Control Unit branch update             & 2                                                           & 2                                                              & 98                                                               & 3743                                                             & 101                                                             & 3969                                                            \\ \hline

08\tikzmark{08d}             & \tikzmark{12}12             & Datapath branch update       & 2                                                           & 0                                                              & 25                                                               & 888                                                              & 20                                                              & 726                                                             \\ \hline

11\tikzmark{11d}             & \tikzmark{13}13             & Control Unit bug fixing                & 6                                                          & 1                                                              & 190                                                              & 5413                                                             & 241                                                             & 8001                                                            \\ \hline

-             & \tikzmark{14}14              & Memory mapped components     & 7                                                          & 0                                                              & 79                                                               & 3079                                                             & 516                                                             & 16237                                                           \\ \hline

-             & 15              & Shift Register bug fix       & 2                                                           & 0                                                              & 38                                                               & 985                                                              & 85                                                              & 2593                                                            \\ \hline

12\tikzmark{12d}              & \tikzmark{16}16            & Datapath bug fixing \& updates    & 6                                                          & 0                                                              & 116                                                              & 2979                                                             & 128                                                             & 4613                                                            \\ \hline

14\tikzmark{14d}             & 17\tikzmark{17}             & Memory mapped constants      & 4                                                           & 0                                                              & 21                                                               & 849                                                              & 101                                                             & 4655                                                            \\ \hline

\tikzmark{03d}03              & \tikzmark{18}18            & ALU optimization                 & 1                                                           & 0                                                              & 2                                                                & 98                                                               & 32                                                              & 1368                                                            \\ \hline \hline 

\multicolumn{3}{|c|}{\textbf{TOTALS}} & 125 & 65 & 1896 & 83916 & 4897 & 206939 \\ \hline
\end{tabular}%
\begin{tikzpicture}[overlay, remember picture, shorten >=.5pt, shorten <=.5pt, transform canvas={yshift=.25\baselineskip}]
    \draw [red,->] ({pic cs:00})  to ({pic cs:00d});
    \draw [red,->] ({pic cs:07})  to ({pic cs:07d});
    \draw [red,->] ({pic cs:08})  to ({pic cs:08d});
    \draw [red,->] ({pic cs:11})  to ({pic cs:11d});
    \draw [red,->] ({pic cs:12})  to ({pic cs:12d});
    \draw [red,->] ({pic cs:14})  to ({pic cs:14d});
    \draw [red,->] ({pic cs:03}) [bend right=20] to ({pic cs:03d});
\end{tikzpicture}
}

==> sec/00preamblelistingsconf.tex <==
\definecolor{mygreen}{rgb}{0,0.6,0}
\definecolor{mygray}{rgb}{0.5,0.5,0.5}
\definecolor{mymauve}{rgb}{0.58,0,0.82}

\makeatletter
\let\old@lstKV@SwitchCases\lstKV@SwitchCases
\def\lstKV@SwitchCases#1#2#3{}
\makeatother
\usepackage{lstlinebgrd}
\makeatletter
\let\lstKV@SwitchCases\old@lstKV@SwitchCases

\lst@Key{numbers}{none}{%
    \def\lst@PlaceNumber{\lst@linebgrd}%
    \lstKV@SwitchCases{#1}%
    {none:\\%
     left:\def\lst@PlaceNumber{\llap{\normalfont
                \lst@numberstyle{\thelstnumber}\kern\lst@numbersep}\lst@linebgrd}\\%
     right:\def\lst@PlaceNumber{\rlap{\normalfont
                \kern\linewidth \kern\lst@numbersep
                \lst@numberstyle{\thelstnumber}}\lst@linebgrd}%
    }{\PackageError{Listings}{Numbers #1 unknown}\@ehc}}
\makeatother

\usepackage{lstlinebgrd} % see http://www.ctan.org/pkg/lstaddons

\makeatletter
\newcommand\notsotiny{\@setfontsize\notsotiny\@vipt\@viipt}
\makeatother

\lstset{
    xleftmargin=10pt,
    xrightmargin=4pt,
    basicstyle=\ttfamily\bfseries\notsotiny,        % the size of the fonts that are used for the code
    breaklines=true,                 % sets automatic line breaking
    commentstyle=\color{mygreen},    % commnt style
    frame=single,	                   % adds a frame around the code
    %framexrightmargin=-5pt,
    keywordstyle=\color{blue},       % keyword style
    numbers=left,                    % where to put the line-numbers; possible values are (none, left, right)
    numbersep=5pt,                   % how far the line-numbers are from the code
    numberstyle=\tiny\color{mygray}, % the style that is used for the line-numbers
    stringstyle=\color{mymauve},     % string literal style
	showstringspaces=false,
    rulecolor=\color{black}
}

